KGATE : a Knowledge Graph Embedding Training Environment

Knowledge graph embedding (KGE) models encode the entities and relations of a knowledge graph into a low-dimensional latent space, enabling tasks such as classification or link prediction. Most KGE models follow an autoencoder architecture, in which an encoder projects the knowledge graph into the latent space and a decoder reconstruct it. Combining both encoder and decoder components is increasingly needed, yet existing libraries rarely support complete autoencoders, are often unmaintained, rely on undocumented default hyperparameters, and produce results that cannot be compared across libraries. Here we present KGATE (Knowledge Graph Autoencoder Training Environment), a modular Python library built on PyTorch Geometric and TorchKGE. KGATE lets users assemble initializers, encoders, decoders, losses, negative samplers, and evaluation metrics as building blocks, or plug in their own block. KGATE includes a preprocessing procedure that controls data leakage, a builtin training pipeline, and reproducibility by design. Benchmarks against six existing KGE libraries show that KGATE training time is comparable with the fastest libraries while offering a broader set of features.

==> hyperref-enhanced.tex <==
\makeatletter
\renewbibmacro*{cite:author}{%
  \iffieldequals{namehash}{\cbx@lasthash}
% Multiple cites in one command
   {\setunit{\compcitedelim}%
    \printtext[bibhyperref]{%
      \usebibmacro{cite:plabelyear+extradate}}}%
% Single cite
   {\printtext[bibhyperref]{%
      \ifnameundef{labelname}
% No author/editor
       {\usebibmacro{cite:noname}%
         \savefield{namehash}{\cbx@lasthash}}
% Normal cite
       {\ifnameundef{shortauthor}
         {\printnames{labelname}}%
         {\cbx@apa@ifnamesaved
            {\printnames{shortauthor}}
            {\printnames[labelname]{author}%
             \addspace\printnames[sabrackets]{shortauthor}}}%
          \savefield{namehash}{\cbx@lasthash}}}}%
   \setunit{\multicitedelim}}

\renewbibmacro*{cite}{%
  \iffieldequals{namehash}{\cbx@lasthash}
% Multiple cites in one command
   {\setunit{\compcitedelim}%
    \printtext[bibhyperref]{%
      \usebibmacro{cite:plabelyear+extradate}}}%
% Single cite
   {\printtext[bibhyperref]{%
      \ifnameundef{labelname}
% No author/editor
       {\usebibmacro{cite:noname}%
         \setunit{\printdelim{nameyeardelim}}%
         \usebibmacro{cite:plabelyear+extradate}%
         \savefield{namehash}{\cbx@lasthash}}
% Normal cite
       {\ifnameundef{shortauthor}
         {\printnames{labelname}}%
         {\cbx@apa@ifnamesaved
           {\printnames{shortauthor}}
           {\printnames[labelname]{author}%
            \addspace\printnames[sabrackets]{shortauthor}}}%
         \setunit{\printdelim{nameyeardelim}}%
        \usebibmacro{cite:plabelyear+extradate}%
        \savefield{namehash}{\cbx@lasthash}}}}%
   \setunit{\multicitedelim}}

\renewbibmacro*{textcite}{%
  \iffieldequals{namehash}{\cbx@lasthash}
% Compact cite - more than one thing for same author
    {\setunit{\compcitedelim}%
     \printtext[bibhyperref]{%
       \usebibmacro{cite:plabelyear+extradate}}}
% New cite
    {\ifbool{cbx:parens}
       {\bibcloseparen\global\boolfalse{cbx:parens}}
       {}%
     \setunit{\textcitedelim}%
     \ifnameundef{labelname}
     % No author/editor
       {\iffieldundef{shorthand}%
    % Cite using title
         {\printtext[bibhyperref]{\usebibmacro{cite:noname}}%
          \setunit{\global\booltrue{cbx:parens}%
                   \printdelim{nonameyeardelim}%
                   \bibopenparen}%
          \printtext[bibhyperref]{%
            \usebibmacro{cite:plabelyear+extradate}}}
    % Cite using shorthand
         {\printtext[bibhyperref]{%
            \usebibmacro{cite:shorthand}}}}
  % Normal cite with author/editor
  % Normal full cite
       {\printtext[bibhyperref]{%
          \ifnameundef{shortauthor}%
    % Normal full cite
           {\printnames{labelname}}
    % Cite using short author
           {\cbx@apa@ifnamesaved
             {\printnames{shortauthor}}
             {\printnames[labelname]{author}}}}%
  % Year
        \setunit{\global\booltrue{cbx:parens}%
                 \printdelim{nameyeardelim}%
                 \bibopenparen}%
  % Put the shortauthor inside the year brackets if necessary
        \printtext[bibhyperref]{%
          \ifnameundef{shortauthor}
           {}
           {\cbx@apa@ifnamesaved
             {}
             {\printnames{shortauthor}%
              \setunit{\printdelim{innernameyeardelim}}}}%
  % Print prenote (belongs to first cite)
        \ifnumequal{\value{citecount}}{1}
           {\usebibmacro{prenote}}
           {}%
  % Actual year printing
        \usebibmacro{cite:plabelyear+extradate}%
  % Save name hash for checks later
        \savefield{namehash}{\cbx@lasthash}}%
    \stepcounter{textcitecount}}}}

\renewbibmacro*{cite:plabelyear+extradate}{%
  \iffieldundef{labelyear}{}
    {\clearfield{labelmonth}% don't want months in citations
     \clearfield{labelday}% don't want days in citations
     \clearfield{labelendmonth}% don't want months in citations
     \clearfield{labelendday}% don't want days in citations
     \clearfield{labelyeardivision}% don't want yeardivisions in citations
     \clearfield{labelendyeardivision}% don't want yeardivisions in citations
     \iffieldsequal{labelyear}{labelendyear}% Don't want no-op year ranges
       {\clearfield{labelendyear}}
       {}%
     \iffieldundef{origyear}
       {}
       {\printorigdate%
        \setunit*{\addslash}}%
     \iffieldundef{related}
       {}
       {\iffieldequalstr{relatedtype}{reprintfrom}
         {\entrydata*{\thefield{related}}{\printlabeldateextra}%
          \setunit*{\addslash}}
         {}}%
     \printlabeldateextra}}

\renewbibmacro*{citeyear}{%
  \iffieldundef{labelyear}
    {\usebibmacro{cite:init}}
    {\iffieldequals{namehash}{\cbx@lasthash}
       {\setunit{\compcitedelim}%
        \printtext[bibhyperref]{\usebibmacro{cite:plabelyear+extradate}}}
       {\printtext[bibhyperref]{\usebibmacro{cite:plabelyear+extradate}}%
        \savefield{namehash}{\cbx@lasthash}}}%
  \setunit{\multicitedelim}}
\makeatother
